OpenMathInstruct-1: A 1.8 Million Math Instruction Tuning Dataset

Recent work has shown the immense potential of synthetically generated datasets for training large language models (LLMs), especially for acquiring targeted skills. Current large-scale math instruction tuning datasets such as MetaMathQA (Yu et al., 2024) and MAmmoTH (Yue et al., 2024) are constructed using outputs from closed-source LLMs with commercially restrictive licenses. A key reason limiting the use of open-source LLMs in these data generation pipelines has been the wide gap between the mathematical skills of the best closed-source LLMs, such as GPT-4, and the best open-source LLMs. Building on the recent progress in open-source LLMs, our proposed prompting novelty, and some brute-force scaling, we construct OpenMathInstruct-1, a math instruction tuning dataset with 1.8M problem-solution pairs. The dataset is constructed by synthesizing code-interpreter solutions for GSM8K and MATH, two popular math reasoning benchmarks, using the recently released and permissively licensed Mixtral model. Our best model, OpenMath-CodeLlama-70B, trained on a subset of OpenMathInstruct-1, achieves a score of 84.6% on GSM8K and 50.7% on MATH, which is competitive with the best gpt-distilled models. We release our code, models, and the OpenMathInstruct-1 dataset under a commercially permissive license.

==> tex/7_conclusion.tex <==
\section{Conclusion}
We introduce \dataset{}, a math instruction tuning dataset with \corrsoln{}M problem-solution pairs with a commercially permissive license.  Compared to previous work, \dataset{} is at least four times bigger. 
The problems are taken from the training set of GSM8K and MATH benchmarks, and the solutions are synthesized by few-shot prompting the Mixtral model. 
With our proposed prompting novelty of using \textit{masked text solutions} and some brute-force scaling, we achieve training set coverage of 99.9\% for the GSM8K benchmark and 93\% for the challenging MATH benchmark. 
The quality of these synthesized solutions is illustrated by finetuning experiments, which show models achieving performance comparable to or outperforming their \textit{gpt-distilled} counterparts.  
To support the open-source efforts in this direction, we publicly release all our fine-tuned models, code, and the \dataset{} along with a further \incorrsoln{}M incorrect sampled solutions.


\section*{Acknowledgement}
We want to thank the NeMo team at NVIDIA for their support. 

